Effect of disorder and doping on electronic structure and diffusion properties of Li$_{3}$V$_{2}$O$_{5}$

V$_{2}$O$_{5}$ in its $\omega$ phase (Li$_{3}$V$_{2}$O$_{5}$) with excess lithium is a potential alternative to the graphite anode for lithium-ion batteries at low temperature and fast charging conditions due to its safer voltage (0.6 V vs Li$^{+}$/Li(s)) and high lithium transport rate. In-operando cationic disorder, as observed in most ordered materials, can produce significant changes in charge compensation mechanisms, anionic activity, lithium diffusion and operational voltages. In this work, we report the variation in structural distortion, electronic structure and migration barrier accompanied by disorder using first-principles calculations. Due to segregation of lithium atoms in the disordered state, we observe greater distortion, emergence of metallic behaviour and potential anionic activity from non-bonding oxygen states near the Fermi level. Redox capacity can be tuned by doping with 3d metals which can adjust the participating cationic states, and by fluorine substitution which can stabilize or suppress anionic states. Moreover, suppression of anionic activity is found to decrease structural distortion, crucial for mitigating voltage fade and hysteresis. Diffusion barrier calculations in the presence of disorder indicate the activation of the remaining 3D-paths for lithium hopping which are unavailable in the ordered configuration, explaining its fast-charging ability observed in experiments.

==> rough.tex <==


\begin{comment}
Following \citet{liu2020disordered}, $\sqrt{2}\times\sqrt{2}\times2$ supercell of primitive rock salt unit cell (\ce{Li6V4O10}) containing 8 formula units of \ce{Li3V2O5} (\ce{Li24V16O40}) was used for OCV calculations and site occupancy of lithium atoms. 
The average voltage can be obtained from the Gibbs free energies of the pristine ($x=0$) and fully-intercalated ($x=2$) structures as 
\begin{eqnarray}
V_{avg} = - \frac{G_{\ce{Li5V2O5}} - G_{\ce{Li3V2O5}} - G_{\ce{Li}(s)}}{e}.
\end{eqnarray}
The open circuit voltage at a given composition ($x=x_{1}$) is simply related to the difference in energy of stable orderings at $x=x_{1}$ and $x = x_{2}$,
\begin{eqnarray}
V = -\frac{G_{\text{Li}_{x_2}\ce{V2O5}} - G_{\text{Li}_{x_1}\ce{V2O5}} - (x_2-x_1)G_{\text{Li}(s)}}{e(x_2-x_1)}.
\end{eqnarray}
Here, $e=-1.602\times10^{-19}$ C is the charge of one electron. The Gibbs free energies were approximated by the DFT single point energies.
\end{comment}

\citet{liu2020disordered} employed this set of disordered pristine structures to identify the most stable configuration as the starting phase for anode and reported open circuit voltages (OCV), site-occupancies and migration barriers using density functional theory (DFT). Using XANES spectra, they showed predominant cationic redox over the anodic range.


In the present work, we explore thermodynamics, kinetics and electronic structure of lesser stable and more distorted orderings of \ce{Li3V2O5} as a potential anode due to the possibility of anionic redox, lower average voltage and improved lithium diffusion pathways. 


Moreover, in contrast to other transition metals (TM), V and Cr based disordered TM\ce{O2} have been reported to possess lower average voltages than their ordered configurations \cite{abdellahi2016understanding}. This property is useful in application as anodes to obtain higher operational voltages, and may be used to tune average voltages and redox capacity with doping.

Fukui function, which is used to visualize charge densities on constituent atoms (to identify redox-active centers) \cite{mccalla2015visualization}, also showed very less localization of charge on oxygen in disordered \ce{Li3V2O5} (S3).
